HYBRIDMIND: Meta Selection of Natural Language and Symbolic Language for Enhanced LLM Reasoning

LLMs approach logical and mathematical reasoning through natural or symbolic languages. While natural language offers human-accessible flexibility but suffers from ambiguity, symbolic reasoning provides precise, machine-executable inferences at the cost of strict domain constraints. We introduce HYBRIDMIND, an adaptive strategy that selects the optimal reasoning approach for each reasoning problem. Through extensive experiments, we evaluate both prompting-based approaches with state-of-the-art LLMs and fine-tuned open-source models. We find that fine-tuning LLaMA-3.1-8B-Instruct as a meta-selector outperforms GPT-4o's natural language reasoning by 4.4\% on FOLIO and 1.3\% on MATH. More notably, using GPT-3.5-turbo as a prompted meta-selector yields a 10\% improvement on FOLIO's challenging subset compared to GPT-4o. We will release our code and data to support future research.

==> table/correct_and_wrong.tex <==
\begin{table}[htbp]
\vspace{-5pt}
    \centering
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        & \multicolumn{2}{c}{PAL} & \multicolumn{2}{c}{COT} \\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & CodeNL & NLCode & CodeNL & NLCode \\ \midrule
        OS incorrect, TS correct & 272 & 243 & 167 & 158 \\
        OS correct, TS incorrect & 80 & 102 & 147 & 189 \\
        \midrule % Adds a horizontal line between the second and third rows
        % Ratio (first row / second row)
        Ratio (first row / second row) & 3.4 & 2.4 & 1.1 & 0.8 \\ 
        \bottomrule
    \end{tabular}
    }
    \label{tab:comparison}
     \caption{Comparison of GPT-4o-mini's performance in one-stage vs. two-stage correctness. 'OS incorrect, TS correct' refers to examples where the model answered incorrectly using only NL or code in one stage but correctly in two stages with a combination of NL and code. Conversely, 'OS correct, TS incorrect' refers to examples where the model answered correctly in one stage using either NL or code, but incorrectly when using the two-stage approach combining NL and code.}
\vspace{-10pt}
\end{table}


==> table/gpt-4o-mini.tex <==
% \begin{table}[htbp]
% \caption{Results of GPT-4o-mini on level-5 problem in MATH dataset}
% \label{tab:gpt-4o-mini}
% \centering
% \setlength{\tabcolsep}{4pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccccccc}
% \toprule
% \textbf{Method} & \textbf{Algebra} & \textbf{Counting \& Probability} & \textbf{Geometry} & \textbf{Number Theory} & \textbf{Intermediate Algebra} & \textbf{Precalculus} & \textbf{Prealgebra} & \textbf{Average} \\
% \midrule
% COT      & 75.57  & 52.85 & 31.06 & 62.99 & 23.57 & 25.93 & 69.43 & 50.60 \\
% PAL      & 47.56  & 46.43 & 18.18 & 56.49 & 16.07 & 10.37 & 57.51 & 36.56 \\
% CodeNL    & \textbf{76.22}  & 54.48 & 28.79 & 68.18 & 23.93 & 21.48 & 69.43 & 50.90 \\
% NLCode   & 66.12  & \textbf{58.54} & 30.30 & \textbf{70.78} & 21.07 & 17.78 & 63.73 & 47.58 \\
% \textbf{MetaMath} & 75.90  & 56.10 & \textbf{32.58} & 64.29 & \textbf{24.64} & 25.19 & \textbf{69.43} & \textbf{51.44} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}
\begin{table*}[htbp]
\centering
\caption{Results of GPT-4o-mini on level-5 problems in the MATH dataset.}
\label{tab:gpt-4o-mini}
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule
\textbf{Method} & \textbf{Algebra} & \textbf{Counting \& Probability} & \textbf{Geometry} & \textbf{Number Theory} & \textbf{Intermediate Algebra} & \textbf{Precalculus} & \textbf{Prealgebra} & \textbf{Average} \\
\midrule
COT      & 75.57  & 52.85 & 31.06 & 62.99 & 23.57 & 25.93 & 69.43 & 50.60 \\
PAL      & 47.56  & 46.43 & 18.18 & 56.49 & 16.07 & 10.37 & 57.51 & 36.56 \\
CodeNL    & \textbf{76.22}  & 54.48 & 28.79 & 68.18 & 23.93 & 21.48 & 69.43 & 50.90 \\
NLCode   & 66.12  & \textbf{58.54} & 30.30 & \textbf{70.78} & 21.07 & 17.78 & 63.73 & 47.58 \\
INC-Math & 75.90  & 56.10 & \textbf{32.58} & 64.29 & \textbf{24.64} & 25.19 & \textbf{69.43} & \textbf{51.44} \\
\midrule
Majority Vote & 83.39  & 60.16 & 30.30 & 77.92 & 26.07 & 20.00 & 75.65 & 55.59 \\
% Oracle Baseline &92.51  &77.24 &49.24 &86.36 &42.86 &38.52 &84.97 &68.96  \\
\midrule
Chosen Accuray &  83.39 & 78.86 &83.33 & 77.92 &81.79 &86.67 &84.46 &82.48 \\
\bottomrule
\end{tabular}%
}
% \vspace{-5pt}
\end{table*}


==> table/gpt-4o-mini_test.tex <==
\usepackage{hyperref}
\begin{table}[htbp]
\vspace{-5pt}
\centering
\caption{Results of GPT-4o-mini on 100 examples in various datasets}
\begin{tabular}{lccc}
\hline
\textbf{Method} & \textbf{GSM8K} & \textbf{Algebra} & \textbf{AIME} \\ 
\hline
COT    & 92             & 88              & 40 (zero-shot) \\ 
PAL    & 87             & 70              & 24 (zero-shot) \\ 
CodeNL & 95             & 93              & 41 (zero-shot) \\ 
NLCode & 91             & 76              & 42 (zero-shot) \\ 
\hline
\end{tabular}
\label{tab:pre_results}
\vspace{-5pt}
\end{table}


==> table/llama3.1-8b.tex <==
\begin{table*}[htbp]
\caption{Results of Llama-3.1-8B-Instruct-Turbo on level-5 problems in the MATH dataset}
\label{tab:llama3.1-8b}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule
\textbf{Method} & \textbf{Algebra} & \textbf{Counting \& Probability} & \textbf{Geometry} & \textbf{Number Theory} & \textbf{Intermediate Algebra} & \textbf{Precalculus} & \textbf{Prealgebra} & \textbf{Average} \\
\midrule
COT      & \textbf{34.53}  & 10.57 & \textbf{6.82} & 18.18 & 4.64 & \textbf{5.19} & \textbf{34.20} & 18.28 \\
PAL      & 15.61  & 7.32 & 1.52 & 14.29 & \textbf{6.43} & 2.22 & 18.65 & 11.71 \\
CodeNL   & 27.69  & 7.32 & 3.79 & 20.13 & 4.29 & 2.96 & 26.42 & 14.88 \\
NLCode   & 31.92  & \textbf{17.07} & 4.55 & \textbf{22.73} & 5.71 & 2.22 & 33.16 & \textbf{18.35} \\
INC-Math & 29.64  & 11.38 & \textbf{6.82} & 19.48 & 5.34 & 2.97 & 30.05 & 16.69 \\
\midrule
MajorityVote & 37.46  & 12.20 & 4.55 & 27.27 & 5.71 & 2.22 & 39.90 & 20.69 \\
% Oracle Baseline & 64.50 & 27.64 &14.39 & 48.05 & 15.71 & 9.63 & 58.55 & 37.39 \\
\midrule
Chosen Accuracy & 65.14 & 83.74 &92.42 &71.43 &89.64 &93.33 &71.50 & 79.31 \\
\bottomrule
\end{tabular}%
}
% \vspace{-5pt}
\end{table*}



==> table/llama3.1-8b_levels.tex <==
\begin{table}[htbp]
\caption{Results for different difficulty levels using LLama 3.1 8B}
\label{tab:llama3.1-8b-levels}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{Level 1} & \textbf{Level 2} & \textbf{Level 3} & \textbf{Level 4} & \textbf{Level 5} \\
\midrule
COT      & 70.71  & 55.15 & 46.42 & 31.22 & 18.13 \\
PAL      & 54.23  & 39.93 & 30.95 & 22.90 & 11.71 \\
CodeNL   & 67.73  & 50.89 & 42.71 & 31.71 & 14.88 \\
NLCode   & 64.30  & \textbf{52.24} & \textbf{45.18} & \textbf{34.84} & \textbf{18.35} \\
\bottomrule
\end{tabular}%
}
\vspace{-5pt}
\end{table}


==> table/number_of_samples.tex <==
\begin{table*}[hbt!]
\centering
\small
\label{tab:math-statistics}
\setlength{\tabcolsep}{1pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 \textbf{Method} 
 & \textbf{Algebra} 
 & \begin{tabular}[c]{@{}c@{}}\textbf{Counting \&}\\\textbf{Probability} \end{tabular} 
 & \textbf{Geometry} 
 & \begin{tabular}[c]{@{}c@{}}\textbf{Number \&}\\\textbf{Theory}\end{tabular} 
 & \begin{tabular}[c]{@{}c@{}}\textbf{Intermediate \&}\\\textbf{Algebra}\end{tabular}
 & \textbf{Precalculus} 
 & \textbf{Prealgebra} 
 & \textbf{Average} \\
\midrule
NL      & \textbf{92.67}	& 78.69 &	\textbf{61.38} &	\underline{81.48} &	58.91 &	\underline{60.07} &	\textbf{89.78}
 & \underline{76.98} \\
\bottomrule
\end{tabular}%
}
\caption{Number of samples in the testing set by categories for MATH.}
\end{table*}

==> table/tokens.tex <==
\begin{table}[htbp]
\vspace{-5pt}
\centering
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{NL} & \textbf{SL} & \textbf{SymbolNL} & \textbf{NLSymbol} & \textbf{INC-Math} \\
\midrule
GPT-4o-mini & 686.20 & 249.68 & 859.22 & 856.25 & 697.99 \\
Llama-3.1-8B & 868.64 & 1136.08 & 1248.17 & 1312.39 & 1119.98 \\
\bottomrule
\end{tabular}%
}
\caption{Average Token Count Comparison: GPT-4o-mini vs. Llama-3.1-8B}
\label{tab:avg_tokens}
\vspace{-5pt}
\end{table}

